Assistive Relative Pose Estimation for On-orbit Assembly using Convolutional Neural Networks

Accurate real-time pose estimation of spacecraft or object in space is a key capability necessary for on-orbit spacecraft servicing and assembly tasks. Pose estimation of objects in space is more challenging than for objects on Earth due to space images containing widely varying illumination conditions, high contrast, and poor resolution in addition to power and mass constraints. In this paper, a convolutional neural network is leveraged to uniquely determine the translation and rotation of an object of interest relative to the camera. The main idea of using CNN model is to assist object tracker used in on space assembly tasks where only feature based method is always not sufficient. The simulation framework designed for assembly task is used to generate dataset for training the modified CNN models and, then results of different models are compared with measure of how accurately models are predicting the pose. Unlike many current approaches for spacecraft or object in space pose estimation, the model does not rely on hand-crafted object-specific features which makes this model more robust and easier to apply to other types of spacecraft. It is shown that the model performs comparable to the current feature-selection methods and can therefore be used in conjunction with them to provide more reliable estimates.

==> ref.tex <==
\begin{thebibliography}{9}
\bibitem{hadaegh-2001}
Beard, R. W., Lawton, J., \& Hadaegh, F. Y. (2001). A coordination architecture for spacecraft formation control. IEEE Transactions on control systems technology, 9(6), 777-790.

\bibitem{hadaegh-2003} 
Scharf, D. P., Hadaegh, F. Y., \& Ploen, S. R. (2003). A survey of spacecraft formation flying guidance and control (part I): Guidance.

\bibitem{hadaegh-2004} 
Scharf, D. P., Hadaegh, F. Y., \& Ploen, S. R. (2004, June). A survey of spacecraft formation flying guidance and control. part ii: control. In Proceedings of the 2004 American control conference (Vol. 4, pp. 2976-2985). IEEE.

\bibitem{damico-2017}
Steindorf, L. M., D’Amico, S., Scharnagl, J., Kempf, F., \& Schilling, K. (2017, February). Constrained low-thrust satellite formation-flying using relative orbit elements. In 27th AAS/AIAA Space Flight Mechanics Meeting.

\bibitem{matsuka-2019}
Matsuka, K., Lupu, E. S., Nakka, Y. K., Foust, R., Chung, S. J., \& Hadægh, F. (2019). Distributed multi-target relative pose estimation for cooperative spacecraft swarm. In: 10th International Workshop on Satellite Constellations and Formation Flying (IWSCFF), 16-19 July 2019, Glasgow, UK. (In Press)

\bibitem{sharma-2018} 
Sharma, S., Beierle, C., \& D'Amico, S. (2018, March). Pose estimation for non-cooperative spacecraft rendezvous using convolutional neural networks. In 2018 IEEE Aerospace Conference (pp. 1-12). IEEE.


\bibitem{capuano-2019} 
Capuano, V., Alimo, S. R., Ho, A. Q., \& Chung, S. J. (2019). Robust Features Extraction for On-board Monocular-based Spacecraft Pose Acquisition. In AIAA Scitech 2019 Forum (p. 2005).

\bibitem{sharma-2018a} S
harma, S., Ventura, J., \& D’Amico, S. (2018). Robust model-based monocular pose initialization for noncooperative spacecraft rendezvous. Journal of Spacecraft and Rockets, 55(6), 1414-1429.

\bibitem{capuano-2019a} 
Capuano, V., Harvard, A., Lin, Y., \& Chung, S. J. (2019). DGNSS-Vision Integration for Robust and Accurate Relative Spacecraft Navigation.

\bibitem{capuano-2020} 
Capuano, V., Kim, K., Harvard, A., \& Chung, S. J. (2020). Monocular-based pose determination of uncooperative space objects. Acta Astronautica, 166, 493-506.

\bibitem{sharma_robust}
Sharma, S., Ventura, J., \& D’Amico, S. (2018). Robust model-based monocular pose initialization for noncooperative spacecraft rendezvous. Journal of Spacecraft and Rockets, 55(6), 1414-1429.

\bibitem{capuano_1} 
Capuano, V., Alimo, S. R., Ho, A. Q., \& Chung, S. J. (2019). Robust Features Extraction for On-board Monocular-based Spacecraft Pose Acquisition. In AIAA Scitech 2019 Forum (p. 2005).


\bibitem{damico-2020}
Park, T. H., Sharma, S., \& D'Amico, S. (2019). Towards Robust Learning-Based Pose Estimation of Noncooperative Spacecraft. arXiv preprint arXiv:1909.00392.

\bibitem{pedro-2019} 
roença, P. F., \& Gao, Y. (2019). Deep Learning for Spacecraft Pose Estimation from Photorealistic Rendering. arXiv preprint arXiv:1907.04298.

\bibitem{damico_dataset-2019}
Kisantal, M., Sharma, S., Park, T. H., Izzo, D., Märtens, M., \& D'Amico, S. (2019). Satellite Pose Estimation Challenge: Dataset, Competition Design and Results. arXiv preprint arXiv:1911.02050.

\bibitem{sharma_pose-2019}
Sharma, S., \& D'Amico, S. (2019). Pose Estimation for Non-Cooperative Rendezvous Using Neural Networks. arXiv preprint arXiv:1906.09868.

% Fridman, L., Brown, D. E., Glazer, M., Angell, W., Dodd, S., Jenik, B., ... & Seaman, S. (2019). MIT advanced vehicle technology study: Large-scale naturalistic driving study of driver behavior and interaction with automation. IEEE Access, 7, 102021-102038.
% ====
\bibitem{pose cnn}
Xiang, Y., Schmidt, T., Narayanan, V., \& Fox, D. (2017). Posecnn: A convolutional neural network for 6d object pose estimation in cluttered scenes. arXiv preprint arXiv:1711.00199.


\bibitem{phoenix darpa}
Sullivan, B., Barnhart, D., Hill, L., Oppenheimer, P., Benedict, B. L., Van Ommering, G., ... \& Will, P. (2013). DARPA phoenix payload orbital delivery system (PODs):“FedEx to GEO”. In AIAA SPACE 2013 conference and exposition (p. 5484).

\bibitem{restore L}
Reed, B. B., Smith, R. C., Naasz, B. J., Pellegrino, J. F., \& Bacon, C. E. (2016). The restore-L servicing mission. In AIAA SPACE 2016 (p. 5478).

\bibitem{deep_features}
Zhou, B., Khosla, A., Lapedriza, A., Oliva, A., \& Torralba, A. (2016). Learning deep features for discriminative localization. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 2921-2929).

\bibitem{surp}
Sonawani, S., Kailas, S., Ben Amor, H., \& Detry, R. Autonomous In-Space Assembly with Arm-Augmented Cubesats. Retrieved from https://interactive-robotics.engineering.asu.edu/autonomous-in-space-assembly-with-arm-augmented-cubesats/.

\bibitem{tracker}
Brahmbhatt, S., Amor, H. B., \& Christensen, H. (2015). Occlusion-Aware Object Localization, Segmentation and Pose Estimation. arXiv preprint arXiv:1507.07882.

\bibitem{roadmaps}
Hall, L. (2015, April 29). 2015 NASA Technology Roadmaps (Archive). Retrieved from https://www.nasa.gov/offices/oct/home/roadmaps/index.html.

\bibitem{Zimpfer}
Zimpfer, D., Kachmar, P., \& Tuohy, S. (2005, January). Autonomous rendezvous, capture and in-space assembly: past, present and future. In 1st Space exploration conference: continuing the voyage of discovery (p. 2523).

\bibitem{Doggett_r}
Doggett, W. (2002, March). Robotic assembly of truss structures for space systems and future research plans. In Proceedings, IEEE Aerospace Conference (Vol. 7, pp. 7-7). IEEE.

\bibitem{langley}
Watson, J. J., Collins, T. J., \& Bush, H. G. (2002, March). A history of astronaut construction of large space structures at McCormick, R., Austin, A., Wehage, K., Backus, S., Miller, R., Leith, J., ... \& Mukherjee, R. (2018, March). REMORA CubeSat for large debris rendezvous, attachment, tracking, and collision avoidance. In 2018 IEEE Aerospace Conference (pp. 1-13). IEEE.


\bibitem{slab}
(n.d.) Retrieved from https://aa.stanford.edu/research/labs-centers/space-rendezvous-laboratory-slab.

\bibitem{cast}
(n.d.). Retrieved from http://cast.caltech.edu/.

\bibitem{coco}
Lin, T. Y., Maire, M., Belongie, S., Hays, J., Perona, P., Ramanan, D., ... \& Zitnick, C. L. (2014, September). Microsoft coco: Common objects in context. In European conference on computer vision (pp. 740-755). Springer, Cham.

\bibitem{openimage}
Kuznetsova, A., Rom, H., Alldrin, N., Uijlings, J., Krasin, I., Pont-Tuset, J., ... \& Ferrari, V. (2018). The open images dataset v4: Unified image classification, object detection, and visual relationship detection at scale. arXiv preprint arXiv:1811.00982.

\bibitem{gazebo}
Koenig, N., \& Howard, A. (2004, September). Design and use paradigms for gazebo, an open-source multi-robot simulator. In 2004 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)(IEEE Cat. No. 04CH37566) (Vol. 3, pp. 2149-2154). IEEE.

\bibitem{ros}
Quigley, M., Conley, K., Gerkey, B., Faust, J., Foote, T., Leibs, J., ... \& Ng, A. Y. (2009, May). ROS: an open-source Robot Operating System. In ICRA workshop on open source software (Vol. 3, No. 3.2, p. 5).


\bibitem{posenet}
Kendall, A., Grimes, M., \& Cipolla, R. (2015). Posenet: A convolutional network for real-time 6-dof camera relocalization. In Proceedings of the IEEE international conference on computer vision (pp. 2938-2946).



\bibitem{sharma cnn}
Sharma, S., Beierle, C., \& D'Amico, S. (2018, March). Pose estimation for non-cooperative spacecraft rendezvous using convolutional neural networks. In 2018 IEEE Aerospace Conference (pp. 1-12). IEEE.
% \bibitem{hess_1} 
% S. R. Alimo, A. Hess, V. Capuano, S. J. Chung, {Convolutional Neural Network For Estimating Satellite Pose From Monocular Images}, CIT File No.: CIT-8090-P, 2018.

\bibitem{imagenet}
Deng, J., Dong, W., Socher, R., Li, L. J., Li, K., \& Fei-Fei, L. (2009, June). Imagenet: A large-scale hierarchical image database. In 2009 IEEE conference on computer vision and pattern recognition (pp. 248-255). Ieee.

\bibitem{vgg}
Simonyan, K., \& Zisserman, A. (2014). Very deep convolutional networks for large-scale image recognition. arXiv preprint arXiv:1409.1556.

\bibitem{alexnet}
Krizhevsky, A., Sutskever, I., \& Hinton, G. E. (2012). Imagenet classification with deep convolutional neural networks. In Advances in neural information processing systems (pp. 1097-1105).

\bibitem{yosinski}
Yosinski, J., Clune, J., Bengio, Y., \& Lipson, H. (2014). How transferable are features in deep neural networks?. In Advances in neural information processing systems (pp. 3320-3328).

\bibitem{geometric loss}
Kendall, A., \& Cipolla, R. (2017). Geometric loss functions for camera pose regression with deep learning. In Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (pp. 5974-5983).


\end{thebibliography}
